Rethinking FUN: Frequency-Domain Utilization Networks

The search for efficient neural network architectures has gained much focus in recent years, where modern architectures focus not only on accuracy but also on inference time and model size. Here, we present FUN, a family of novel Frequency-domain Utilization Networks. These networks utilize the inherent efficiency of the frequency-domain by working directly in that domain, represented with the Discrete Cosine Transform. Using modern techniques and building blocks such as compound-scaling and inverted-residual layers we generate a set of such networks allowing one to balance between size, latency and accuracy while outperforming competing RGB-based models. Extensive evaluations verifies that our networks present strong alternatives to previous approaches. Moreover, we show that working in frequency domain allows for dynamic compression of the input at inference time without any explicit change to the architecture.

==> additional_fun_experiments.tex <==
\section{Additional FUN Experiments} \label{additional_fun_experiments}
\subsection{Input Compression} \label{input compression section}
\begin{table}
    \setlength{\tabcolsep}{2.2pt}
    \centering
    \resizebox{1.0\columnwidth}{!}{ 
    \begin{tabular}{c c c c c}
    \toprule
    \# Input Channels & Y/Cb/Cr & Top-1 Acc. & \# Parameters (M) \\
    \midrule
    $192$ &
    \multicolumn{1}{c}{$64/64/64$} &
    \multicolumn{1}{c}{$77.01$} &
    \multicolumn{1}{c}{$4.23$}  \\ 
    $88$ & 
    \multicolumn{1}{c}{$64/12/12$} &
    \multicolumn{1}{c}{$76.02$} &
    \multicolumn{1}{c}{$3.99$} \\
    $88$ &
    \multicolumn{1}{c}{$44/22/22$} &
    \multicolumn{1}{c}{$74.15$} &
    \multicolumn{1}{c}{$3.99$} \\
    $64$ & 
    \multicolumn{1}{c}{$44/10/10$} &
    \multicolumn{1}{c}{$73.95$} &
    \multicolumn{1}{c}{$3.96$}   \\
    $48$ & 
    \multicolumn{1}{c}{$32/8/8$} &
    \multicolumn{1}{c}{$69.45$} &
    \multicolumn{1}{c}{$3.93$}   \\
    $24$ & 
    \multicolumn{1}{c}{$14/5/5$} &
    \multicolumn{1}{c}{$51.85$} &
    \multicolumn{1}{c}{$3.91$} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Effects of dropping channels on accuracy and model size for EFNet-B0}
\label{tb:performace_vs_num_channels}
\end{table}

\begin{figure}
    \includegraphics[scale=0.4]{figures/fig_input_compression.png}
    \caption{Imagenet Acc vs input compression ratio}
    \label{imagenet_acc_vs_input_compression}
\end{figure}


In this experiment, we take a trained eFUN show the effects of discarding input channels on the model accuracy and size. To do so, during inference we zero out selected Y, Cb, and Cr channels. 
We show that one can significantly reduce the number of frequency channels used to represent the input by keeping only the lowest frequency channels in each of Y, Cb, and Cr.

Our results, presented in Table~\ref{tb:performace_vs_num_channels}, show that when using our FUN framework, one can significantly reduce the size of the input, while maintaining a relatively high accuracy. For example, dropping $54\%$ of the input channels (from $192$ to $88$) results in a $1\%$ drop in accuracy while dropping $75\%$ of the input channels results in a $7.5\%$ drop in accuracy. These results offer a desirable property: as no additional training is performed here, our framework inherently supports different possible operating points with regard to the input compression ratio. 

% As an RGB-based alternative to the compression shown above on DCT inputs, we propose down-sampling the RGB-represented image along it's spatial dimensions. We then proceed and evaluate the trained model's accuracy on the down-sampled images for different compression factors. The results, shown in Figure~\ref{imagenet_acc_vs_input_compression}, show that RGB-based networks are much more sensitive to input compression compared to the FUN-based model and suffer a very large performance drop even when compressing by a factor of only $2$.

\begin{table}
    \setlength{\tabcolsep}{2.2pt}
    \centering
    \resizebox{1.0\columnwidth}{!}{ 
    \begin{tabular}{c c c}
    \toprule
    Model & Imagenet Top-1 Acc.& \# Parameters(M)\\
    \midrule
    eFUN &
    \multicolumn{1}{c}{77} &
    \multicolumn{1}{c}{4.2} \\ 
    DCT-Encoder &
    \multicolumn{1}{c}{72.8} &
    \multicolumn{1}{c}{4.3} \\ 
    Learned-DCT &
    \multicolumn{1}{c}{77.2} &
    \multicolumn{1}{c}{4.3} \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{comparison of jpeg dct vs learnable transforms}
\label{tb:res_learnable_dct}
\end{table}

\begin{figure*}
\setlength{\tabcolsep}{1pt}
\centering
    \begin{tabular}{c c c}
        \includegraphics[width=0.3\textwidth]{figures/fig_learnable_dct_finetune.png}&
        \includegraphics[width=0.3\textwidth]{figures/fig_learnable_dct_full_train.png}&
        \includegraphics[width=0.3\textwidth]{figures/fig_dct.png}
    \end{tabular}
    \caption{dct filters. Left to right: learned encoder, learned full train, static JPEG \yac{This names are not clear, but I assume we'll fix that later.}}
    \label{fig:dct_filers}
\end{figure*}

\subsection{A Learnable DCT Transformation}
In this experiment, we study whether the input DCT can be replaced with a learnable convolutional layer. In particular, the new convolutional layer receives as input a YCbCr image obtained from its RGB representation. It then transforms each $8\times8\times1$ input block into $1\times1\times64$ outputs. The final DCT output, of size $28\times28\times192$, is then fed into the original network, as before.

We propose two methods of learning this transformation:
\begin{enumerate}
    \item Adding a DCT-like convolutional layer before the eFUN architecture and training the entire network end-to-end, denoted Learnable-DCT
    \item Adding a DCT-like convolutional layer before an already trained eFUN model and training only the added convolutional layer, denoted DCT-Encoder.
\end{enumerate}
Intuitively, the second approach implements an "encoder-decoder" architecture, where the decoder is a fixed eFUN network and the encoder is trained to produce inputs similar to those expected by the decoder.

The results achieved by each of the methods are presented in Table~\ref{tb:res_learnable_dct}. We can see that using the learned convolutional filters provides the best accuracy, while being a slightly larger model compared to the standard eFUN model.
% (Since it doesn't have the learn-able transformation layer). 
Freezing the entire network with the exception of the input convolutional layer results poor accuracy. However, by allowing the entire network to learn, the Learnable-DCT method achieves accuracy slightly higher than that of our eFUN model.

The filters learned by each of the three methods are presented in Figrue~\ref{fig:dct_filers}. We can see that some of the filters learned by our new layers seem similar to those of the standard DCT - they include vertical and horizontal lines in some frequency. However, most filters still look rather different than those of the DCT, showing the usefulness of using the static DCT filters, which allow us a level of understanding and a built-in meaningful ordering of the filters, which does not exist for the learned filters. \yac{I am not sure what is supposed to be better, but seems like the right-most is the nicest. Need to see how we can formulat that to make it standout?} \kgc{I tried explaining a bit more}

Our results show that using a DCT-like learned convolutional layer for RGB inputs can provide results similar to those of eFUN models in terms of model size, latency, and top-1 accuracy. However, using a learned transformation makes it difficult to analyze the importance of each input channel and does not provide inherent support for dynamic input compression presented in Section~\ref{input compression section}.

==> discussion.tex <==
\section{Discussion} \label{Discussion}
1. Frequency domain is good for smaller models

2. Wider inputs allow shallower networks which speed up inference

3. FLOPs isn't a good measure for GPU latency

4. Frequency domain is a built-in way of prioritizing input information, unlike just resizing the RGB input image

5. With some prior knowledge on the data (e.g. - natural images usually don't feature high frequencies) efficiency can be leveraged further

6. Room for more research - NAS, architectures for less channels, optimizing for CPU, other transforms
